Differentially Private Optimal Power Flow for Distribution Grids

Although distribution grid customers are obliged to share their consumption data with distribution system operators (DSOs), a possible leakage of this data is often disregarded in operational routines of DSOs. This paper introduces a privacy-preserving optimal power flow (OPF) mechanism for distribution grids that secures customer privacy from unauthorised access to OPF solutions, e.g., current and voltage measurements. The mechanism is based on the framework of differential privacy that allows to control the participation risks of individuals in a dataset by applying a carefully calibrated noise to the output of a computation. Unlike existing private mechanisms, this mechanism does not apply the noise to the optimization parameters or its result. Instead, it optimizes OPF variables as affine functions of the random noise, which weakens the correlation between the grid loads and OPF variables. To ensure feasibility of the randomized OPF solution, the mechanism makes use of chance constraints enforced on the grid limits. The mechanism is further extended to control the optimality loss induced by the random noise, as well as the variance of OPF variables. The paper shows that the differentially private OPF solution does not leak customer loads up to specified parameters.

==> figures/opf_figure.tex <==
\begin{figure}
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tikzpicture}[
    PV_node/.style={circle,scale=0.75,color=black,fill=black},
    font=\scriptsize,
    ]
    % sets
    \draw [gray!50,line width = 0.02cm, fill=gray!30,fill opacity=0.2] (-0.25,2.0) -- (-0.25,3.15) -- (3.75,3.15) -- (3.75,2.0) -- (-0.25,2.0);
    \draw [gray!50,line width = 0.02cm, fill=gray!30,fill opacity=0.2] (-0.7,1.5) -- (-0.7,3.45) -- (3.85,3.45) -- (3.85,1.5) -- (-0.7,1.5);
    % \draw [gray!50,line width = 0.02cm, fill=gray!30,fill opacity=0.2] (4.75,4.15) -- (5.75,4.15) -- (5.75,1.15) -- (4.75,1.15) -- (4.75,4.15);
    \draw [gray!50,line width = 0.02cm, fill=gray!30,fill opacity=0.2] (4.75,4.15) -- (7.25,4.15) -- (7.25,1.0) -- (4.75,1.0) -- (4.75,4.15);
    % nodes
    \node[PV_node,label=above:{$0$}] (n0) at (0.0,2.5) {};
    \node[PV_node,label=above:{$i-1$}] (ni_1) at (1.75,2.5) {};
    \node[PV_node,label=above:{$i$}] (ni) at (3.5,2.5) {};
    \node[PV_node,label=above:{$i+1$}] (ni+1) at (5.25,3.5) {};
    \node[PV_node,label=above:{$i+2$}] (ni+2) at (5.25,1.5) {};
    \node[PV_node,label=above:{}] (ni+11) at (7.0,3.5) {};
    \node[PV_node,label=above:{}] (ni+21) at (7.0,1.5) {};
    \node[PV_node,label=above:{}] (ni_2) at (2.5,1.75) {};
    % lines
    \draw[black,line width=0.025cm] (n0) -- (0.5,2.5);
    \draw[black,dotted,line width=0.025cm] (0.5,2.5) -- (1.25,2.5);
    \draw[black,line width=0.025cm] (1.25,2.5) -- (ni_1);
    \draw[black,line width=0.025cm] (ni_1) -- (ni);
    \draw[black,line width=0.025cm] (ni) -- (ni+1);
    \draw[black,line width=0.025cm] (ni) -- (ni+2);
    \draw[black,line width=0.025cm] (ni+1) -- (5.75,3.5);
    \draw[black,dotted,line width=0.025cm] (5.75,3.5) -- (6.5,3.5);
    \draw[black,line width=0.025cm] (6.5,3.5) -- (ni+11);
    \draw[black,line width=0.025cm] (ni+2) -- (5.75,1.5);
    \draw[black,dotted,line width=0.025cm] (5.75,1.5) -- (6.5,1.5);
    \draw[black,line width=0.025cm] (6.5,1.5) -- (ni+21);
    \draw[black,line width=0.025cm] (ni_1) -- (1.75,2.0);
    \draw[black,dotted,line width=0.025cm] (1.75,2.0) -- (1.75,1.75);
    \draw[black,dotted,line width=0.025cm] (1.75,1.75) -- (2.0,1.75);
    \draw[black,line width=0.025cm] (2.0,1.75) -- (2.5,1.75);
    % node power
    \draw [black,->,>=stealth,line width = 0.02cm] (2.45,2.65) -- (3.1,2.65) node[above,midway]{$f_{i}^{\dag}$};
    \draw [black,->,>=stealth,line width = 0.02cm] (3.5,2.25) -- (3.5,1.75) node[below]{$d_{i}^{\dag}$};
    \draw [black,->,>=stealth,line width = 0.02cm] (3.5,3.5) node[above]{$g_{i}^{\dag}$} -- (3.5,3.0);
    \draw[black,line width=0.02cm,->,>=stealth] (4.0,2.95) -- node[above,midway,sloped]{$f_{i+1}^{\dag}$} (4.5,3.25);
    \draw[black,line width=0.02cm,->,>=stealth] (4.0,2.05) -- node[below,midway,sloped]{$f_{i+2}^{\dag}$} (4.5,1.75);
    % set labels
    \draw[gray!50,line width=0.02cm,fill=white] (4.75,1.0) circle (0.225cm) node{\textcolor{black}{$\set{D}_{i}$}};
    % \draw[gray!50,line width=0.02cm,fill=white] (4.75,1.15) circle (0.25cm) node{\textcolor{black}{$\set{C}_{i}$}};
    \draw[gray!50,line width=0.02cm,fill=white] (-0.7,3.45) circle (0.225cm) node{\textcolor{black}{$\set{U}_{i}$}};
    \draw[gray!50,line width=0.02cm,fill=white] (-0.25,2.0) circle (0.225cm) node{\textcolor{black}{$\set{R}_{i}$}};
    \end{tikzpicture}
}
\caption{Topology of the distribution grid relative to node $i$, $\dag=\{p,q\}$.}
\label{grid_topology}
\end{figure}


==> figures/opf_proj.tex <==
% \begin{figure}
%     \centering
%     \resizebox{0.38\textwidth}{!}{%
%     \begin{tikzpicture}
%     % objective function
%     % projections
%     % \draw[step=.5,gray,thin] (0,0) grid (6,3);
%     \draw[gray, densely dotted, line width = 0.02cm] (0.75,1.75) -- (2.4,1.75);
%     \draw[gray, densely dotted, line width = 0.02cm] (1.35,0.4) -- (2.65,0.4);
%     \draw[gray, densely dashed] (1.48,1.48) -- (1.48,0);
%     \draw[gray, densely dashed] (1.48,1.48) -- (2.7,1.48);
%     \draw[gray, densely dashed] (2.01,1.0) -- (2.01,0);
%     \draw[gray, densely dashed] (2.01,.96) -- (4.5,0.96);
%     \draw[gray,<-,>=stealth] (1.48,0.1) -- (2.01,0.1);
%     \node[draw=none,font=\scriptsize,scale=0.9] at (1.75,0.25) {$\textcolor{black}{\Theta}$};
%     \begin{axis}[
%     font=\scriptsize,
%     ymin=2.5,
%     ymax=15,
%     xmin=0,
%     xmax=30,
%     no markers, 
%     domain=-30:30, 
%     samples=300,
%     separate axis lines,
%     axis lines = middle,
%     axis y line*=right,
%     axis x line shift=-0 pt,
%     xlabel={operating cost}, 
%     ylabel={$s$}, 
%     xlabel style={yshift=-0.45cm,xshift=-0.5cm,font=\scriptsize,scale=0.85},
%     ylabel style={yshift=0.1cm,xshift=-0.4cm,scale=0.9},
%     x dir=reverse,
%     height=4cm, 
%     width=4cm,
%     xtick=\empty,
%     ytick=\empty,
%     enlargelimits=false]
%     % cost function
%     \addplot+[name path = plot,domain=4.5:11.5,line width = 0.025cm,black] ({(x-7.5)^2+5},{x});
%     \addplot+[domain=11.5:12.44,line width = 0.01cm,black,densely dashed] ({(x-7.5)^2+5},{x});
%     \addplot+[domain=3.0:4.5,  line width = 0.01cm,black,densely dashed] ({(x-7.5)^2+5},{x});
%     % feasibility space
%     \addplot+[name path=yaxis,domain=4.5:11.5,line width = 0.07cm,maincolor] ({0},{x});
%     \addplot[black] coordinates {(2.5,10.9)} node[scale=0.9]{$\textcolor{maincolor}{\set{S}}$};
%     % power flow solutions
%     \addplot[black] coordinates {(5,7.5)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]190:{$s^{\star}$}},scale=0.85]{\tiny\textcolor{maincolor}{\faStar}};
%     \addplot[black] coordinates {(11.5,10.1)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]190:{$\tilde{s}$}},scale=0.85]{\tiny\textcolor{maincolor}{\faCircle}};
%     % fill the feasibility area
%     \addplot[maincolor!20] fill between[of=yaxis and plot,reverse=true];
%     \end{axis}
%     % power flow
%     \begin{axis}[
%     xshift=2.4cm,
%     font=\scriptsize,
%     ymin=2.5,
%     ymax=15,
%     xmin=0,
%     xmax=0.325,
%     no markers, 
%     % domain=-30:30, 
%     samples=301,
%     separate axis lines,
%     axis lines = middle,
%     axis y line*=left,
%     hide y axis,
%     axis x line shift=-0 pt,
%     xlabel={probability density}, 
%     xlabel style={xshift=-0.35cm,yshift=-0.45cm,font=\scriptsize,scale=0.85},
%     height=4cm, 
%     width=4cm,
%     xtick=\empty,
%     ytick=\empty,
%     enlargelimits=false]
%     \addplot+[domain=3.0:11.5,line width = 0.025cm,black] ({gauss(7.5,1.4)},{x});
%     \addplot[black] coordinates {(0.05,9.0)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]25:{$\mathbb{P}[\tilde{s}\in\textcolor{maincolor}{\set{S}}]$}}]{};
%     % \node[coordinate,pin={[pin edge={blue,ultra thick}]left:{A pin!} } ]
%         % at (axis cs:4,54.59815) {};
%     \addplot[black] coordinates {(-0.0075,4.15)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]0:{$\mathbb{P}[\tilde{s}\notin\textcolor{maincolor}{\set{S}}]$}}]{};
%     % fill the left side of pdf        
%     \addplot [name path = plot, draw=none, domain=11.5:4.5] ({gauss(7.5,1.4)},{x});
%     \addplot+[name path=yaxis,domain=4.5:11.5,draw=none] ({0},{x});
%     \addplot[maincolor!20] fill between[of=yaxis and plot,reverse=false];
%     % fill the right side of pdf  
%     \addplot [name path = plot2, draw=none, domain=0:4.5] ({gauss(7.5,1.4)},{x});
%     \addplot+[name path=yaxis2,domain=4.5:0,draw=none] ({0},{x});
%     \addplot[red!80] fill between[of=yaxis2 and plot2,reverse=false];
%     \addplot[domain=4.5:0,draw=black] ({0},{x});
%     \end{axis}
%     \end{tikzpicture}
%     }
%     \caption{Projections of OPF solutions onto operating cost and feasibility space.}
%     \label{OPF_projections}
% \end{figure}



\begin{figure}
    \centering
    \hspace{1.5cm}\resizebox{0.3\textwidth}{!}{%
    \begin{tikzpicture}
    % objective function
    % projections
    % \draw[step=.5,gray,thin] (0,0) grid (6,3);
    % \draw[gray, densely dotted, line width = 0.02cm] (0.75,1.75) -- (2.4,1.75);
    % \draw[gray, densely dotted, line width = 0.02cm] (1.35,0.4) -- (2.65,0.4);
    
    
    % horizontal dashed lines
    \draw[gray, densely dashed] (0.135,1.04) -- (3.45,1.04);
    \draw[gray, densely dashed] (0.8,0.68) -- (2.2,0.68);
    % vertical dashed lines
    \draw[gray, densely dashed] (0.8,0.68) -- (0.8,1.45);
    \draw[gray, densely dashed] (0.135,1.04) -- (0.135,1.45);
    \draw[gray,->,>=stealth] (0.8,1.35) -- (0.135,1.35);
    \node[draw=none,font=\scriptsize,scale=0.8] at (0.475,1.45) {$\textcolor{black}{\Theta}$};
    \begin{axis}[
    xshift=-1.2cm,
    font=\scriptsize,
    ymin=-2.5,
    ymax=17,
    xmin=0,
    xmax=60,
    no markers, 
    domain=-30:30, 
    samples=300,
    separate axis lines,
    % axis lines = middle,
    axis y line*=right,
    axis lines = middle,
    axis x line*=bottom,
    axis x line shift=-0 pt,
    xlabel={operating cost}, 
    ylabel={$s$}, 
    xlabel style={yshift=-0.75cm,xshift=0.6cm,font=\scriptsize,scale=0.8},
    ylabel style={xshift=-0.4cm,scale=1},
    x dir=reverse,
    height=4cm, 
    width=4cm,
    xtick=\empty,
    ytick=\empty,
    enlargelimits=false]
    % cost function
    \addplot+[name path = plot,domain=2.0:12,line width = 0.025cm,black] ({(1.25*x-3.5)^2+10},{x});
    \addplot+[domain=10.5:13.5,line width = 0.01cm,black,densely dashed] ({(1.25*x-3.5)^2+10},{x});
    \addplot+[domain=-2.0:4.5,  line width = 0.01cm,black,densely dashed] ({(1.25*x-3.5)^2+10},{x});
    % feasibility space
    \addplot+[name path=yaxis,domain=2.0:12,line width = 0.07cm,maincolor] ({0},{x});
    \addplot[black] coordinates {(5,10.9)} node[scale=0.9]{$\textcolor{maincolor}{\set{S}}$};
    % power flow solutions
    \addplot[black] coordinates {(10,3.2)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]190:{$s^{\star}$}},scale=0.85]{\tiny\textcolor{maincolor}{\faStar}};
    \addplot[black] coordinates {(27,6.1)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]190:{$\tilde{s}$}},scale=0.85]{\tiny\textcolor{maincolor}{\faCircle}};
    % fill the feasibility area
    \addplot[maincolor!20] fill between[of=yaxis and plot,reverse=true];
    \end{axis}
    % power flow
    \begin{axis}[
    xshift=1.2cm,
    font=\scriptsize,
    ymin=-2.5,
    ymax=20,
    xmin=0,
    xmax=0.325,
    no markers, 
    % domain=-30:30, 
    samples=301,
    separate axis lines,
    % axis lines = middle,
    axis y line*=left,
    axis lines = middle,
    hide y axis,
    axis x line*=bottom,
    xlabel={probability density}, 
    xlabel style={yshift=-0.75cm,xshift=-0.45cm,font=\scriptsize,scale=0.8},
    height=4cm, 
    width=4cm,
    xtick=\empty,
    ytick=\empty,
    enlargelimits=false]
    \addplot+[domain=-1:15,line width = 0.025cm,black,xshift=-0.05cm] ({2*gauss(7.1,2.6)},{x});
    \addplot[black] coordinates {(0.05,10.0)} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]25:{$\mathbb{P}[\tilde{s}\in\textcolor{maincolor}{\set{S}}]$}}]{};
    \addplot[black] coordinates {(-0.0001,2.5 )} node[pin={[pin edge={blue,line width = 0.015 cm},scale=0.9]350:{$\mathbb{P}[\tilde{s}\notin\textcolor{maincolor}{\set{S}}]$}}]{};
    % % fill the left side of pdf        
    \addplot [name path = plot, domain=2.7:15,xshift=-0.05cm,draw=none] ({2*gauss(7.1,2.6)},{x});
    \addplot+[name path=yaxis,  domain=15:2.7,draw=none] ({0},{x});
    \addplot[maincolor!20] fill between[of=yaxis and plot,reverse=false];
    % % fill the right side of pdf  
    \addplot [name path = plot2, draw=none, domain=-1:2.7,xshift=-0.05cm] ({2*gauss(7.1,2.6)},{x});
    \addplot+[name path=yaxis,  domain=2.7:-1,draw=none] ({0},{x});
    \addplot[red!80] fill between[of=yaxis and plot2,reverse=false];
    \addplot[domain=2.7:-2.5,draw=black, line width = 0.015cm] ({0},{x});
    \end{axis}
    \end{tikzpicture}
    }
    \caption{Projections of OPF solutions onto operating cost and feasibility space.}
    \label{OPF_projections}
\end{figure}




